Pervasive Label Errors in Test Sets Destabilize Machine Learning Benchmarks

We identify label errors in the test sets of 10 of the most commonly-used computer vision, natural language, and audio datasets, and subsequently study the potential for these label errors to affect benchmark results. Errors in test sets are numerous and widespread: we estimate an average of at least 3.3% errors across the 10 datasets, where for example label errors comprise at least 6% of the ImageNet validation set. Putative label errors are identified using confident learning algorithms and then human-validated via crowdsourcing (51% of the algorithmically-flagged candidates are indeed erroneously labeled, on average across the datasets). Traditionally, machine learning practitioners choose which model to deploy based on test accuracy - our findings advise caution here, proposing that judging models over correctly labeled test sets may be more useful, especially for noisy real-world datasets. Surprisingly, we find that lower capacity models may be practically more useful than higher capacity models in real-world datasets with high proportions of erroneously labeled data. For example, on ImageNet with corrected labels: ResNet-18 outperforms ResNet-50 if the prevalence of originally mislabeled test examples increases by just 6%. On CIFAR-10 with corrected labels: VGG-11 outperforms VGG-19 if the prevalence of originally mislabeled test examples increases by just 5%. Test set errors across the 10 datasets can be viewed at https://labelerrors.com and all label errors can be reproduced by https://github.com/cleanlab/label-errors.

==> Makefile <==
.PHONY: main clean FORCE

main: paper.pdf abstract.txt

paper.pdf: FORCE
	latexmk -pdflatex='pdflatex -interaction nonstopmode' -pdf paper.tex

clean:
	latexmk -pdf -C
	rm -f abstract.txt

%.txt: %.tex
	pandoc $< -o $@ -f latex -t plain --wrap=none


.PHONY: spell
spell: $(shell find . -name '*.tex')
	$(eval SPELLTEX := $(shell sh ./bin/get-tex-files.sh paper.tex))
	@ for i in $(SPELLTEX); do aspell -l en_us --mode=tex \
					  --add-tex-command="autoref p" \
					  --add-tex-command="Cref p" \
					  --add-tex-command="crefformat pp" \
					  --add-tex-command="tikzstyle p" \
					  --add-tex-command="usetikzlibrary p" \
					  --add-tex-command="settopmatter p" \
					  --add-tex-command="lstdefinelanguage pp" \
					  --add-tex-command="lstdefinestyle pp" \
					  --add-tex-command="setlist op" \
					  --add-tex-command="setitemize p" \
					  --add-tex-command="definecolor ppp" \
					  --add-tex-command="color p" \
					  --add-tex-command="newcommand pp" \
					  -p ./aspell.words -c $$i; done
	@ for i in $(SPELLTEX); do perl bin/double.pl $$i; done
	@ bash bin/hyphens.sh $(SPELLTEX)
	@ ( head -1 aspell.words ; tail -n +2 aspell.words | LC_ALL=C sort ) > aspell.words~
	@ mv aspell.words~ aspell.words
.PHONY: spell

